Debiased inference for a covariate-adjusted regression function

In this article, we study nonparametric inference for a covariate-adjusted regression function. This parameter captures the average association between a continuous exposure and an outcome after adjusting for other covariates. In particular, under certain causal conditions, this parameter corresponds to the average outcome had all units been assigned to a specific exposure level, known as the causal dose-response curve. We propose a debiased local linear estimator of the covariate-adjusted regression function, and demonstrate that our estimator converges pointwise to a mean-zero normal limit distribution. We use this result to construct asymptotically valid confidence intervals for function values and differences thereof. In addition, we use approximation results for the distribution of the supremum of an empirical process to construct asymptotically valid uniform confidence bands. Our methods do not require undersmoothing, permit the use of data-adaptive estimators of nuisance functions, and our estimator attains the optimal rate of convergence for a twice differentiable function. We illustrate the practical performance of our estimator using numerical studies and an analysis of the effect of air pollution exposure on cardiovascular mortality.

==> theorems.tex <==
\clearpage
\section{Conditions}

Here, we re-state the conditions we use in our asymptotic results for convenience. These are the same conditions as stated in the main text.
\begin{enumerate}[label=\textbf{(A\arabic*)}]
\item \label{cond:bounded_K} The kernel $K$ is a mean-zero, symmetric, nonnegative, and Lipschitz continuous density function with support contained in $[-1,1]$. Additionally, $K$ belongs to the linear span of the functions whose subgraph can be represented as a finite number of Boolean operations among sets of the form $\{(s,u) \in \d{R} \times \d{R} : p(s,u) \leq \varphi(u)\}$ where $p$ is a polynomial and $\varphi$ is an arbitrary real function. 
\item \label{cond:bandwidth} As $n \longrightarrow \infty$, the bandwidths $h = h_n$ and $b = b_n$ satisfy $h_n \longrightarrow 0$,  $nh_n \longrightarrow \infty$, and $\tau_n := h_n/b_n \longrightarrow \tau \in (0,\infty)$.
\end{enumerate}

We define the following pseudo-distance for any $P_0$-square integrable functions $\gamma_1, \gamma_2 : \s{A} \times \s{W} \to \mathbb{R}$, $\s{A}_0 \subset \s{A}$, and $\s{S} \subseteq \s{A} \times \s{W}$:
\begin{align*}
    d(\gamma_1, \gamma_2; \s{A}_0, \s{S}) :=  \sup_{a \in \s{A}_0} \left\{E_0 [I_{\s{S}}(a,W)\{\gamma_1(a,W) - \gamma_2(a,W)\}^2]\right\}^{1/2}
\end{align*}
We also define $B_\varepsilon(a_0)$ as the closed ball of radius $\varepsilon$ centered at $a_0$. 

\begin{enumerate}[label=\textbf{(A\arabic*)}]
\setcounter{enumi}{2}
    \item \label{cond:uniform_entropy_nuisances} There exist classes of functions $\s{F}_\mu$ and $\s{F}_g$ such that almost surely for all $n$ large enough, $\mu_0, \mu_n \in \s{F}_\mu$, $g_0,g_n \in \s{F}_g$, and for some constants $C_j\in (0, \infty)$, $V_\mu \in (0,1)$, and $V_g \in (0,2)$:
        \begin{enumerate}
            \item \label{cond:bounded_cond} $|\mu| \leq C_1$ for all $\mu \in \s{F}_\mu$, and $C_2 \leq g \leq C_3$ for all $g \in \s{F}_g$;
            \item \label{cond:entropy_cond} $ \sup_Q \log N(\varepsilon, \s{F}_\mu, L_2(Q)) \leq C_4 \varepsilon^{-V_\mu}$ and $\sup_Q \log N(\varepsilon, \s{F}_g, L_2(Q)) \leq C_5  \varepsilon^{-V_g}$ for all $\varepsilon > 0$.
        \end{enumerate}
    \item \label{cond:doubly_robust} There exist $\mu_\infty \in \s{F}_\mu$ and $g_\infty \in \s{F}_g$, $\delta_1 > 0$, and subsets $\s{S}_1, \s{S}_2$ and $\s{S}_3$ of $B_{\delta_1}(a_0)\times \s{W}$ such that $\s{S}_1 \cup \s{S}_2 \cup \s{S}_3 = B_{\delta_1}(a_0)\times \s{W}$ and:
        \begin{enumerate}
            \item $\mu_\infty(a, w) = \mu_0(a, w)$ for all $(a, w) \in \s{S}_1 \cup \s{S}_3$ and $g_\infty(a, w) = g_0(a, w)$ for all $(a,  w) \in \s{S}_2 \cup \s{S}_3$;
            \item $d(\mu_n,\mu_\infty; B_{\delta_1}(a_0),\s{S}_1) = \fasterthan\left( \{nh\}^{-1/2}\right)$, and $d(g_n,g_\infty; B_{\delta_1}(a_0),\s{S}_1) = \fasterthan(1)$;
            \item $d(g_n,g_\infty; B_{\delta_1}(a_0),\s{S}_2)\} = \fasterthan\left( \{nh\}^{-1/2}\right)$, and $d(\mu_n,\mu_\infty; B_{\delta_1}(a_0),\s{S}_1) = \fasterthan(1)$;
            \item $d(\mu_n,\mu_\infty; B_{\delta_1}(a_0),\s{S}_3)d(g_n,g_\infty; B_{\delta_1}(a_0),\s{S}_3) = \fasterthan\left( \{nh\}^{-1/2}\right)$.
        \end{enumerate}
    \item \label{cond:cont_density} It holds that:
    \begin{enumerate}
        \item $\theta_0$ is twice continuously differentiable on $B_{\delta_1}(a_0)$;
        \item $f_0$ is positive and Lipschitz continuous on $B_{\delta_1}(a_0)$; 
        \item there exist $\delta_2 > 0$ and $C_6 < \infty$ such that $E_0[|Y|^{2+\delta_2} \mid A = a, W = w] \leq C_6$ for all $a \in B_{\delta_1}(a_0)$ and $P_0$-almost every $w$ and $E_0[ |Y|^4] < \infty$; and 
        \item $a \mapsto \sigma_0^2(a) := E_0\left[ \{\xi_\infty(Y,A,W) - \theta_0(A)\}^2 \mid A = a\right]$ is bounded and continuous on $B_{\delta_1}(a_0)$, where $\xi_\infty := \xi_{\mu_\infty, g_\infty, Q_0}$ is the limiting pseudo-outcome.
    \end{enumerate}
\end{enumerate}



Let $\s{A}_0$ be a compact subset of $\s{A}$ over which we wish to perform uniform inference. For $\delta > 0$ define $\s{A}_\delta$ as the $\delta$-enlargement of $\s{A}_0$; that is, the set of $a \in \d{R}$ such that there exists $a_0 \in \s{A}_0$ with $|a - a_0| \leq \delta$. We then assume there exists $\delta_3 > 0$ such that the following hold.



\begin{enumerate}[label=\textbf{(A\arabic*)}]\setcounter{enumi}{5}
    \item \label{cond:unif_nuisance_rate}The constant $V := \max\{V_\mu, V_g\}$, for $V_\mu$ and $V_g$ defined in~\ref{cond:uniform_entropy_nuisances} and the bandwidth $h$  satisfies $n\left[ h / (\log n)\right]^{\frac{2+V}{2-V}} \longrightarrow \infty$ and $nh^3 \longrightarrow \infty$.
    \item \label{cond:unif_doubly_robust} There exist $\mu_\infty \in \s{F}_\mu$, $g_\infty \in \s{F}_g$, $\delta_3 > 0$ and subsets $\s{S}_1', \s{S}_2'$, and $\s{S}_3'$ of $\s{A}_{\delta_3}\times \s{W}$ such that $\s{S}_1' \cup \s{S}_2' \cup \s{S}_3' = \s{A}_{\delta_3}\times \s{W}$ and:
        \begin{enumerate}
            \item $\mu_\infty(a, w) = \mu_0(a, w)$ for all $(a, w) \in \s{S}_1' \cup \s{S}_3'$ and $g_\infty(a, w) = g_0(a, w)$ for all $(a,  w) \in \s{S}_2' \cup \s{S}_3'$;
            \item $d(\mu_n,\mu_\infty; \s{A}_{\delta_3},\s{S}_1') = \fasterthan\left( \{nh \log n\}^{-1/2}\right)$;
            \item $d(g_n,g_\infty; \s{A}_{\delta_3},\s{S}_2')\} = \fasterthan\left( \{nh \log n\}^{-1/2}\right)$;
            \item $d(\mu_n,\mu_\infty; \s{A}_{\delta_3},\s{S}_3)d(g_n,g_\infty; \s{A}_{\delta_3},\s{S}_3) = \fasterthan\left( \{nh \log n\}^{-1/2}\right)$.
            \item $d(\mu_n,\mu_\infty; \s{A}_{\delta_3},\s{A} \times \s{W})$ and $d(g_n,g_\infty; \s{A}_{\delta_3},\s{A} \times \s{W})$ are both $\fasterthan\left(h^{\frac{V}{2(2-V)}}\{\log n\}^{-\frac{1}{2-V}}\right)$
        \end{enumerate}
    \item \label{cond:holder_smooth_theta} It holds that:
    \begin{enumerate}
        \item $\theta_0$ is twice continuously differentiable with H\"{o}lder-continuous second derivative on $\s{A}_{\delta_3}$; 
        \item $f_0$ is Lipschitz continuous and bounded away from 0 and $\infty$ on $\s{A}_{\delta_3}$;
        \item $|Y|$ is $P_0$-almost surely bounded; and
        \item  $a \mapsto E_0\left[ \{\xi_\infty(Y,A,W) - \theta_0(A)\}^2 \mid A = a\right]$ is continuous on $\s{A}_{\delta_3}$.
    \end{enumerate}
\end{enumerate}
